Universal Vision-Language Dense Retrieval: Learning A Unified Representation Space for Multi-Modal Retrieval

This paper presents Universal Vision-Language Dense Retrieval (UniVL-DR), which builds a unified model for multi-modal retrieval. UniVL-DR encodes queries and multi-modality resources in an embedding space for searching candidates from different modalities. To learn a unified embedding space for multi-modal retrieval, UniVL-DR proposes two techniques: 1) Universal embedding optimization strategy, which contrastively optimizes the embedding space using the modality-balanced hard negatives; 2) Image verbalization method, which bridges the modality gap between images and texts in the raw data space. UniVL-DR achieves the state-of-the-art on the multi-modal open-domain question answering benchmark, WebQA, and outperforms all retrieval models on the two subtasks, text-text retrieval and text-image retrieval. It demonstrates that universal multi-modal search is feasible to replace the divide-and-conquer pipeline with a united model and also benefits single/cross modality tasks. All source codes of this work are available at https://github.com/OpenMatch/UniVL-DR.

==> Section/limitation.tex <==
\section*{Limitations}
VL-UnivSearch focuses on encoding multi-modality sources in a universal embedding space for retrieval. However, there are also some limitations left for future research to explore. The queries in the WebQA dataset are only annotated to be related to texts or images, leading to some biases during evaluation. Even though the captions are effective to represent images, the caption descriptions inevitably contain noises and can be missed in the Web search, which may limit the multi-modality retrieval performance and our image verbalization methods via query generation.

==> Table/ablation.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{minipage}[c]{0.45\textwidth}
\centering
\small
\resizebox{\linewidth}{!}{%
    \begin{tabular}{l|ccc}
    \hline
    \multirow{2}[0]{*}{\textbf{Model}}  & \multicolumn{3}{c}{\textbf{Retrieval Performance}} \\ \cline{2-4}
     & Text & Image & Multi \\\hline
    \multicolumn{4}{l}{\textit{Single Modality Models}} \\\hline
    %BM25 & 62.17 & 57.89 & 53.75 \\
    BERT-DPR  & 37.09 & 52.34 & - \\
    VinVL-DPR w/o caption & - & 3.67  & - \\
    VinVL-DPR w/o img feature  & - & 51.56 & - \\
    VinVL-DPR & 25.00 & 48.68 & - \\
    CLIP-DPR w/o caption & - & 17.74 & - \\
    CLIP-DPR w/o img feature  & - & 58.17 & - \\
    CLIP-DPR & 52.57 & 59.95 & - \\\hline
    \multicolumn{4}{l}{\textit{Universal Multi-Modality Models}} \\\hline
    VinVL-DPR w/o img feature & 29.01 & 46.55 & 36.13 \\
    VinVL-DPR & 29.95 & 49.65 & 38.14 \\
    %+ img expansion & 50.87 & 51.36 & 53.37 \\\hline
    CLIP-DPR w/o img feature & 51.47 & 57.36 & 50.33 \\
    CLIP-DPR  & 51.75 & 60.61  & 48.83 \\
    VL-UnivSearch & \textbf{60.91} & \textbf{65.61}  & \textbf{62.54} \\\hline
    
    %+ img expansion & 59.72 & 60.14 & 63.12 \\\hline
    %\multicolumn{4}{l}{\textit{Multi-Modality w. Hard Negative Training}} \\\hline
    %VinVL w. caption & 55.80 & 56.16 & 56.42 \\
    %+ img feature & 49.65 & 50.19 & 52.26 \\
    %+ img expansion & 60.95 & 61.29 & 61.31 \\\hline
    %CLIP w. caption & 62.29 & 62.64 & 64.66 \\
    %+ img feature  & 65.20 & 65.51 & 67.59 \\
    %+ img expansion  & \textbf{65.69} & \textbf{65.99} & \textbf{67.98} \\\hline
    \end{tabular}}
    \caption{Retrieval Performance of Different Ablation Models. MRR@10 is used as the evaluation metric.}
  \label{tab:ablation}%
\end{minipage}

==> Table/hard_neg_exp.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[h]
  \centering
      \small
      \resizebox{\linewidth}{!}{%
    \begin{tabular}{l}
    \hline
    \textbf{Figures}\\\hline
	\hline

    \end{tabular}}
  \caption{Image Verbalization Cases. We highlight the matching phrases between user queries and manual captions or image verbalization results.}
  \label{tab:}%
\end{table*}%


==> Table/hard_negs.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
% Table generated by Excel2LaTeX from sheet 'Sheet1'

\begin{minipage}[c]{0.45\textwidth}
\centering
\resizebox{\linewidth}{!}{%
    \begin{tabular}{l|ccc|r}
    \hline
    \multirow{2}{*}{\textbf{Sampling}}  & \multicolumn{3}{c|}{\textbf{Retrieval Performance}}  & \textbf{Retrieved} \\\cline{2-4}
     & Text & Image & Multi & \textbf{Image} (\%) \\\hline
    \multicolumn{5}{l}{\textit{Inbatch Training}} \\\hline
    DPR (Random) & 51.67 & 60.60 & 48.73 & 26.82 \\
    Balanced Inbatch & 52.24  & 59.99  & 49.88 & 30.35 \\\hline
    \multicolumn{5}{l}{\textit{Hard Negative Training}} \\\hline
    %Only Texts   & 57.26  & 55.20  & 38.94  & 89.89  \\
    %Only Images    & 55.39  & \textbf{67.25}  & 35.10  & 2.81  \\
    %More Texts     & 58.49  & 64.88  & 61.12  & 49.33  \\
    %More Images    & 57.83  & 65.66  & 61.21  & 48.12  \\
    %Inbatch Random & 58.09 & 65.73 & 61.34 & 48.57\\\hline
    %Balance   &  \textbf{58.61}  & 65.58  &  \textbf{61.43}  & 49.36  \\\hline
    Only Texts   & 54.92 & 52.88  & 36.26  &  91.74\\
    Only Images    & 55.85 & \textbf{66.51}  & 33.49  & 1.97 \\
    2 Texts \& 1 Image   & 59.18 & 65.15  & 61.64  &  49.53  \\
    1 Text \& 2 Images   & 57.86 & 66.23 & 61.20  &  47.88 \\
    ANCE (Random) & 59.85 & 64.80 & 61.72 & 50.01 \\\hline
    Balanced Inbatch   &  \textbf{60.58} & 65.21 & \textbf{62.29} & 49.11 \\\hline
    \end{tabular}}
     \caption{Effectiveness of Different Hard Negative Training Strategies. These hard negative trained models start from inbatch trained ones and are contisuously fine-tuned with different numbers of hard negatives. The MRR@10 score and the image ratio of Top 10 retrieved candidates are shown to evaluate retrieval effectiveness.}
  \label{tab:hardneg}%
\end{minipage}




==> Table/image_results.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
  \small
  
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|ccc}
    \hline
    \textbf{Model} & \textbf{MRR@10} & \textbf{MRR@20} & \textbf{NDCG@20} \\\hline
    \multicolumn{4}{l}{\textit{Single Modality Training}} \\\hline
    BERT  & 52.34 & 52.84 & 54.94 \\
    VinVL w/o caption & 3.67  & 4.03  & 5.55 \\
    VinVL w/o img feature  & 51.56 & 52.10  & 54.16 \\
    VinVL & 48.68 & 49.16 & 51.38 \\
    CLIP w/o caption & 17.74 & 18.53 & 21.98 \\
    CLIP w/o img feature  & 58.17 & 58.70  & 61.46 \\
    CLIP & 59.95 & 60.38 & 63.61 \\\hline
    \multicolumn{4}{l}{\textit{Multi-Modality Training}} \\\hline
    VinVL w/o img feature & 46.55 & 47.15 & 49.41 \\
    VinVL & 49.65 & 50.19 & 52.26 \\
    %+ img expansion & 50.87 & 51.36 & 53.37 \\\hline
    CLIP w/o img feature & 57.36 & 57.85 & 60.55 \\
    CLIP  & 60.60  & 61.03 & 63.59 \\
    VL-UnivSearch & \textbf{65.69}  & \textbf{65.99}  & \textbf{67.98} \\\hline
    %+ img expansion & 59.72 & 60.14 & 63.12 \\\hline
    %\multicolumn{4}{l}{\textit{Multi-Modality w. Hard Negative Training}} \\\hline
    %VinVL w. caption & 55.80 & 56.16 & 56.42 \\
    %+ img feature & 49.65 & 50.19 & 52.26 \\
    %+ img expansion & 60.95 & 61.29 & 61.31 \\\hline
    %CLIP w. caption & 62.29 & 62.64 & 64.66 \\
    %+ img feature  & 65.20 & 65.51 & 67.59 \\
    %+ img expansion  & \textbf{65.69} & \textbf{65.99} & \textbf{67.98} \\\hline
    \end{tabular}}
    \caption{Image Retrieval Performance of Different Vision-Language Models.}
  \label{tab:ablation_img}%
\end{table}%


==> Table/image_verbalization_raw.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
  \small
    \begin{tabular}{l|ccc}
    \hline
   \multirow{2}[0]{*}{\textbf{Model}} & \multicolumn{3}{c}{\textbf{Retrieval Performance}} \\ \cline{2-4}
          & Text & Image & Muti \\\hline
    \multicolumn{4}{l}{\textit{Inbatch Training}} \\\hline
    VL-UnivSearch  &  51.75 & 60.61  & 48.83   \\
    w. Verbalized Caption  & 51.51  & 60.57  & 49.49  \\
    w. Verbalized Query & \textbf{52.14}  & 59.72  & \textbf{50.21}  \\\hline
    \multicolumn{4}{l}{\textit{Balanced Hard Negative Training}} \\\hline
    %VL-UnivSearch  & 58.61  & \textbf{65.58}  & 61.43  \\
    %w. Verbalized Caption & 59.36  & 65.38  & 61.55  \\
    %w. Verbalized Query & \textbf{59.45} & 65.20  & \textbf{61.73}  \\\hline
    VL-UnivSearch & 60.58 & 65.21 & 62.29  \\
    w. Verbalized Caption & 59.86  & \textbf{65.87}  & 62.24  \\
    w. Verbalized Query & \textbf{60.91} & 65.61  & \textbf{62.54}  \\\hline
    \end{tabular}%
      \caption{Performance of Multi-Modality Retrieval Models with Different Image Verbalization Methods. All models are evaluated with MRR@10.}
  \label{tab:img_verb_performance}%
\end{table}%

==> Table/imbalance_negs.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
  \small
    \begin{tabular}{l|ccc}
    \hline
   \multirow{2}[0]{*}{\textbf{Sampling}} & \multicolumn{3}{c}{\textbf{Retrieval Performance}} \\ \cline{2-4}
          & Text & Image & Muti \\\hline
    %\multicolumn{4}{l}{\textit{Imbalanced Sampling}} \\\hline
    %VL-UnivSearch (Inbatch) & 51.67  & 60.60  & 48.73  \\
    %\multicolumn{4}{l}{\textit{Imbalanced Hard Negative Training}} \\\hline
    %VL-UnivSearch (Imbalanced)  & 59.80  & 64.78 &  61.87 \\
    %w. Verbalized Caption & 59.91 & 65.20 & 62.10 \\
    Inbatch Random  & 60.26 & 65.31 & 62.21  \\
    %\multicolumn{4}{l}{\textit{Balanced Sampling}} \\\hline
    %VL-UnivSearch (Inbatch) & 52.24  & 59.99  & 49.88  \\
    %VL-UnivSearch (Balanced) & 60.09 & 64.71 & 61.86 \\
    %w. Verbalized Caption & 59.93 & 64.98 & 61.65 \\
    Balance & \textbf{60.67} & \textbf{65.54} & \textbf{62.41} \\\hline
    \end{tabular}%
      \caption{Performance of Multi-Modality Retrieval Models with Different Image Verbalization Methods. All models are evaluated with MRR@10.}
  \label{tab:img_verbalization}%
\end{table}%

==> Table/overall.tex <==

\begin{table*}

  \small
  \centering
    \begin{tabular}{l|l|ccc|ccc}
    \hline
    \textbf{Training} & \textbf{Model} & \textbf{MRR@10} & \textbf{NDCG@10} & \textbf{Rec@10} & \textbf{MRR@20} & \textbf{NDCG@20} & \textbf{Rec@20} \\
    \hline
    - &  BM25  & 53.75 & 49.60  & 61.06 & 54.10  & 51.72 & 68.16 \\
    \hline
    \multirow{3}[0]{*}{Zero Shot}  & CLIP w. img caption & 18.16 & 16.76 & 22.90  & 18.60  & 18.27 & 27.97 \\
    & CLIP w. img feature & 10.59 & 8.69  & 11.65 & 10.80  & 9.52  & 14.32 \\ 
    & DPR & 22.72 & 20.06 & 27.00 & 23.14 & 21.79 & 32.78 \\ \hline
     Inbatch & DPR & 41.88 & 39.65 & 52.61 & 42.44 & 42.35 & 61.71 \\
     %& bm25 Inbatch neg & 47.39 & 44.54 & 57.75 & 47.91 & 47.18 & 66.63 \\
     Hard Neg & DPR &  45.54 & 42.05 & 52.45 & 45.93 & 43.83 & 58.42 \\\hline
    \multirow{3}[0]{*}{Inbatch} & VinVL w. img caption & 36.13 & 33.48 & 43.17 & 36.72 & 35.82 & 51.09 \\
         
    & + img feature & 38.14 & 35.43 & 45.91 & 38.74 & 37.79 & 53.89 \\
    & + caption expansion & 39.13 & 36.37 & 46.91 & 39.66 & 38.67 & 54.70 \\
          \hline
          
     \multirow{3}[0]{*}{Hard Neg} & VinVL w. img caption & 41.86 & 38.55 & 47.84 & 42.23 & 40.08 & 53.00 \\
     & + img feature & 42.29 & 39.06 & 48.88 & 42.68 & 40.70  & 54.40 \\
     & + caption expansion &  45.12 & 41.54   &  50.89 &  45.50 & 43.16 & 56.34 \\\hline
       
    \multirow{3}[0]{*}{Inbatch} & CLIP w. img caption & 50.33 & 47.27 & 60.66 & 50.81 & 49.83 & 69.21 \\
    & + img feature & 48.73 & 46.27 & 60.44 & 49.24 & 49.06 & 69.83 \\
    & + caption expansion & 50.21 & 47.51 & 61.65 & 50.71 & 50.28 & 70.99 \\\hline
     \multirow{3}[0]{*}{Hard Neg}     & CLIP w. img caption & 59.58 & 56.25 & 70.35 & 59.89 & 58.38 & 77.43 \\
   & + img feature & 61.53 & 58.17 & 72.07 & 61.81 & 60.04 & 78.23 \\
    
    & + caption expansion & \textbf{61.82} & \textbf{58.60}  & \textbf{72.89} & \textbf{62.11} & \textbf{60.57} & \textbf{79.38} \\\hline
    \end{tabular}
    \caption{Overall Performance.}
  \label{tab:overall}
\end{table*}


==> Table/text_results.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
  \small
  
  \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{l|ccc}
    \hline
    \textbf{Model} & \textbf{MRR@10} & \textbf{MRR@20} & \textbf{NDCG@20} \\\hline
    \multicolumn{4}{l}{\textit{Single Modality Training}} \\\hline
    BERT  & 37.09 & 37.70  & 34.42 \\
    VinVL & 25.00 & 25.57 & 22.85 \\
    CLIP  & 52.57 & 52.96 & 49.50 \\\hline
    \multicolumn{4}{l}{\textit{Multi-Modality Training}} \\\hline
    VinVL w/o img feature & 29.01 & 29.60  & 26.01 \\
    VinVL & 29.95 & 30.59 & 26.69 \\
    %+ img expansion & 30.47 & 30.96 & 27.23 \\\hline
    CLIP w/o img feature & 51.47 & 51.84 & 48.21 \\
    CLIP  & 51.67 & 52.05 & 48.45 \\
    VL-UnivSearch & \textbf{59.00}  & \textbf{59.28}  & \textbf{54.07} \\\hline
    %+ img expansion  & 52.14 & 52.50  & 48.75 \\\hline
    %\multicolumn{4}{l}{\textit{Multi-Modality w. Hard Negative Training}} \\\hline
    %VinVL w. caption & 28.14 & 22.35 & 23.89 \\
    %+ img feature & 29.14 & 29.55 & 24.69 \\
    %+ img expansion & 29.68 & 30.13 &25.34 \\\hline
    %CLIP w. caption & 58.12 & 58.39 & 53.10 \\
    %+ img feature  & \textbf{59.02} & 59.25 & 53.47 \\
    %+ img expansion  & 59.00 & \textbf{59.28} & \textbf{54.07} \\\hline
    \end{tabular}}
    \caption{Text Retrieval Performance of Different Vision-Language Models.}
  \label{tab:ablation_text}
\end{table}%

